Learning Exponential Families in High-Dimensions: Strong Convexity and Sparsity

The versatility of exponential families, along with their attendant convexity properties, make them a popular and effective statistical model. A central issue is learning these models in high-dimensions, such as when there is some sparsity pattern of the optimal parameter. This work characterizes a certain strong convexity property of general exponential families, which allow their generalization ability to be quantified. In particular, we show how this property can be used to analyze generic exponential families under L_1 regularization.

==> new.tex <==
@article{vandeGeer08,
	author = {Sara A. van de Geer},
	title = {High-dimensional generalized linear models and the lasso},
	journal = {Annals of Statistics},
	volume = {36},
	number = {2},
	pages = {614--645},
	year = {2008}
}

@article{Bunea08,
	author = {Florentina Bunea},
	title = {Honest variable selection in linear and logistic regression models via $\ell_1$ and $\ell_1+\ell_2$ penalization},
	journal = {Electronic Journal of Statistics},
	volume = {2},
	year = {2008},
	pages = {1153--1194}
}

@article{Bach09,
  author    = {Francis Bach},
  title     = {Self-concordant analysis for logistic regression},
  journal   = {CoRR},
  volume    = {abs/0910.4627},
  year      = {2009},
  note      = {{\tt http://arxiv.org/abs/0910.4627}}
}

@inproceedings{NegahbanRaWaYu09,
	author = {S. Negahban and P. Ravikumar and M. Wainwright and B. Yu},
	title = {A unified framework for high-dimensional analysis of M-estimators with decomposable regularizers},
	booktitle = {NIPS},
	year = {2009}
}

@ARTICLE{MeinshausenYu,
  author = {Nicolai Meinshausen and Bin Yu},
  title = {Lasso-type recovery of sparse representations for high-dimensional data},
  journal = {Annals of Statistics},
  volume = {37},
  pages = {246},
  year = {2009}
} 


@article{bickel-2008,
  author = {Peter J. Bickel and Ya'acov Ritov and Alexandre B. Tsybakov},
  title = {Simultaneous analysis of {L}asso and {D}antzig selector},
  journal = {Annals of Statistics},
  volume = {37},
  number = {4},
  pages = {1705--1732},
  year = {2008}
}

@ARTICLE{candes-2007-35,
  author = {Emmanuel Candes and Terence Tao},
  title = {The {D}antzig selector: Statistical estimation when $p$ is much larger   than $n$},
  journal = {Annals of Statistics},
  volume = {35},
  pages = {2313},
  year = {2007}
}


@techreport{Ravikumar:1141507,
      author       = "Ravikumar, Pradeep and Wainwright, Martin J and Raskutti,
                      Garvesh and Yu, Bin",
      title        = "High-dimensional covariance estimation by minimizing
                      l1-penalized log-determinant divergence",
      number       = "arXiv:0811.3628",
      month        = "Nov",
      year         = "2008",
 }

@techreport{Ravikumar:Ising,
      author       = "Ravikumar, P. and Wainwright, M. J. and Lafferty, J.",
      title        = "High-dimensional Ising model selection using l1-regularized logistic regression.",
      number       = "Technical Report 750, UC Berkeley, Department of Statistics.",
      year         = "2008",
 }

@article{ghosal,
 author = {Ghosal, Subhashis},
 title = {Asymptotic normality of posterior distributions for exponential families when the number of parameters tends to infinity},
 journal = {J. Multivar. Anal.},
 volume = {74},
 number = {1},
 year = {2000},
 issn = {0047-259X},
 pages = {49--68},
 publisher = {Academic Press, Inc.},
 address = {Orlando, FL, USA},
 }

@article{portnoy,
 author = {S. Portnoy},
 title = {Asymptotic behavior of likelihood methods for exponential families when the number of parameters tends to infinity.},
 journal = {Annals of Statistics},
 volume = {16},
 year = {1988}
 }


